Multi-Modal Mutual Information (MuMMI) Training for Robust Self-Supervised Deep Reinforcement Learning

This work focuses on learning useful and robust deep world models using multiple, possibly unreliable, sensors. We find that current methods do not sufficiently encourage a shared representation between modalities; this can cause poor performance on downstream tasks and over-reliance on specific sensors. As a solution, we contribute a new multi-modal deep latent state-space model, trained using a mutual information lower-bound. The key innovation is a specially-designed density ratio estimator that encourages consistency between the latent codes of each modality. We tasked our method to learn policies (in a self-supervised manner) on multi-modal Natural MuJoCo benchmarks and a challenging Table Wiping task. Experiments show our method significantly outperforms state-of-the-art deep reinforcement learning methods, particularly in the presence of missing observations.

==> sections/pushingresults.tex <==
\begin{table*}[hbt!]
\centering
\caption{\small Box Pushing Performance measured by Mean Total Episodic Reward (averaged over 30 episodes, with standard deviations). Highest average reward in \textbf{bold}.}
\label{tbl:CSResults_Pushing}
\small  
\begin{tabular}{c c c c }
\hline
\hline 
    Modalities & MuMMI & MuMMI-b & MSSM-e \\
\hline
    All Modalities (Medium Missing Data)  & $\mathbf{-17.8}\pm20.0$ & $-19.0\pm23.2$ & $-34.1\pm25.7$ \\
    
    All Modalities (Full Observed)  & $\mathbf{-12.3}\pm6.4$ & $-12.7\pm10.1$ & $-31.7\pm20.1$ \\
    

    Robot Camera (Medium Missing Data) & $-15.3\pm9.5$ & $\mathbf{-13.2}\pm7.9$ & $-29.1\pm15.2$ \\ 

    Robot Camera (Full Observed)
    & $\mathbf{-14.1}\pm8.8$ & $-15.1\pm7.2$ & $-27.7\pm14.6$ \\ 

\hline
\hline
\end{tabular}
    \vspace{-0.3cm}
\end{table*}
